Dynamic Kernel Graph Sparsifiers

A geometric graph associated with a set of points $P= \{x_1, x_2, \cdots, x_n \} \subset \mathbb{R}^d$ and a fixed kernel function $\mathsf{K}:\mathbb{R}^d\times \mathbb{R}^d\to\mathbb{R}_{\geq 0}$ is a complete graph on $P$ such that the weight of edge $(x_i, x_j)$ is $\mathsf{K}(x_i, x_j)$. We present a fully-dynamic data structure that maintains a spectral sparsifier of a geometric graph under updates that change the locations of points in $P$ one at a time. The update time of our data structure is $n^{o(1)}$ with high probability, and the initialization time is $n^{1+o(1)}$. Under certain assumption, our data structure can be made robust against adaptive adversaries, which makes our sparsifier applicable in iterative optimization algorithms. We further show that the Laplacian matrices corresponding to geometric graphs admit a randomized sketch for maintaining matrix-vector multiplication and projection in $n^{o(1)}$ time, under sparse updates to the query vectors, or under modification of points in $P$.

==> 62_impact.tex <==
% \section{Broader Impact}
% \label{sec:impact}
% Our algorithms enhance the efficiency of real-time updates in geometric graphs, benefiting applications in network analysis, machine learning, and computational geometry, and potentially influencing various fields requiring dynamic graph processing.

\section{Impact Statement}
\label{sec:impact}
This paper presents work whose goal is to advance the field of Machine Learning. Our algorithms enhance the efficiency of real-time updates in geometric graphs, benefiting applications in network analysis, machine learning, and computational geometry, and potentially influencing various fields requiring dynamic graph processing. This is a theoretical work. As far as we are aware, our work does not have negative societal impact. 
